CPU frequency scheduling of real-time applications on embedded devices with temporal encoding-based deep reinforcement learning

Small devices are frequently used in IoT and smart-city applications to perform periodic dedicated tasks with soft deadlines. This work focuses on developing methods to derive efficient power-management methods for periodic tasks on small devices. We first study the limitations of the existing Linux built-in methods used in small devices. We illustrate three typical workload/system patterns that are challenging to manage with Linux's built-in solutions. We develop a reinforcement-learning-based technique with temporal encoding to derive an effective DVFS governor even with the presence of the three system patterns. The derived governor uses only one performance counter, the same as the built-in Linux mechanism, and does not require an explicit task model for the workload. We implemented a prototype system on the Nvidia Jetson Nano Board and experimented with it with six applications, including two self-designed and four benchmark applications. Under different deadline constraints, our approach can quickly derive a DVFS governor that can adapt to performance requirements and outperform the built-in Linux approach in energy saving. On Mibench workloads, with performance slack ranging from 0.04 s to 0.4 s, the proposed method can save 3% - 11% more energy compared to Ondemand. AudioReg and FaceReg applications tested have 5%- 14% energy-saving improvement. We have open-sourced the implementation of our in-kernel quantized neural network engine. The codebase can be found at: https://github.com/coladog/tinyagent.

==> author.tex <==
\author{\IEEEauthorblockN{
Ti Zhou,
Jueqi Wang,
Man Lin
% Student Two\IEEEauthorrefmark{2}, 
% Student Three\IEEEauthorrefmark{3}
}

\IEEEauthorblockA{
Department of Computer Science, \\
St. Francis Xavier University, Nova Scotia, Canada \\
% Email: x2019cwm@stfx.ca
% \IEEEauthorrefmark{2}
% \IEEEauthorrefmark{2}studentTwo,
% \IEEEauthorrefmark{3}studentThree@student.mdh.se
}}


==> sections/acknowledgement.tex <==
\section*{Acknowledgment}
The authors would like to thank ... for his/her/their help and support during the process of writing this paper. \cite{webpage, FundConDep,exampleofjournalarticle,exampleofconferencepaper}

==> sections/keywords.tex <==
\begin{center}
\begin{IEEEkeywords}
CPU, energy consumption measurement
\end{IEEEkeywords}
\end{center}


==> sections/linux.tex <==
\section{\textcolor{cyan}{Limitations of short-term system feature based DVFS strategies: }}   

As of V 5.13, Linux offers six DVFS policies: \textit{Performance, Powersave, Userspace, Ondemand, Conservative and Schedutil}. They are called Linux CPUFreq governors.
\textit{Performance} and \textit{Powersave} fixed the frequency at the highest/lowest value, respectively.
\textit{Userspace} leaves the frequency adjustment to the user-space.

\textit{Ondemand, Conservative and Schedutil} are three governors that run in the kernel state and dynamically adjust the CPU frequency.
\textit{Ondemand} and \textit{Conservative} are time triggered. 
They use a timer to regularly sample information from the past period and control the frequency of the next period.
\textit{Schedutil}, which is the newest governor, is implemented as part of the scheduler. It does not rely on a timer, but is actively woken up by the scheduler to tune the frequency. 

\subsection{Heuristic-Based Linux Built-In Governors}

\begin{algorithm}
\label{algo:ondemand}
\caption{\textit{Ondemand} DVFS governor in Linux V5.13: a simplified description}
\begin{algorithmic}[1]

\State $F$ denotes the provided frequency options.
\State $min_f/max_f$ denotes the min/max supported frequency in $F$.
\State $next_f$ denotes the frequency to be applied.

\For{each sampling period}
  \State Calculate the last period's CPU utilization $u$, $u \in [0, 1]$.
  
  \If {$u > up\_threshold$ (tunable, $\in [0, 1]$, 0.8 by default)}
    \State $next_f = max_f$.
  \Else
    \State $next_f = min_f + (max_f - min_f) \times u$.
  \EndIf
  
  \State $next_f = (1 - powersave\_bias$(tunable, $\in [0, 1]$, 0 by default)$) \times next_f$.
  \State $next_f$ = the highest frequency below or at $next_f$ supported in $F$.
  \State Apply $next_f$.
 
\EndFor

\end{algorithmic}
\end{algorithm}

The built-in governors are designed to handle general situations.
They are expected to run at high frequencies. For most nowadays consumer laptops, the \textit{Ondemand} governor will run 100 times a second with the default \cite{cpufreqdoc}.
Algorithm 1 describes the summary of \textit{Ondemand} in Linux V5.13.
\textit{Schedutil}'s core strategy is similar to \textit{Ondemand}, they differ in the implementation way and the utilization metric. \textit{Schedutil} is part of the scheduler, and the tuning depends on the scheduling class invoking its utilization update callback for that CPU, e.g., it doesn't have a regular tuning interval.
For \textit{Ondemand} and \textit{Conservative}, utilization (also known as load) is characterized as the percentage of time that a CPU is actually running the workload.
\textit{Schedutil} uses another metric: Per Entity Load Tracking (PELT) provided by scheduler context to calculate utilization.

If the utilization is greater than a threshold, \textit{Ondemand} will immediately turn the frequency to the maximum (lines 6-7 in algorithm 1).
Otherwise \textit{Ondemand} will pick a frequency proportional to the utilization (line 9 in algorithm 1).

For \textit{Ondemand} and \textit{Schedutil}, meeting performance is the primary objective.
\textit{Conservative} does not immediately raise or lower the frequency, but increases or decreases at a fixed pace.
In practice, \textit{Conservative} tends to lose more performance and save more energy.
With the default settings, \textit{Ondemand} and \textit{Schedutil} can all be seen as attempts to save energy with as little performance loss as possible.
When we want to purposefully tune the trade off between energy and performance in a aggressive way, only Ondemand provides such support (via \textit{powersave\_bias}) \cite{cpufreqdoc}.

We show a profiling of \textit{Ondemand} in real operation (visualization is showed in Fig.~\ref{fig:4}). The hardware environment is a Nvidia Jetson Nano Board 2GB.
This workload is a periodic face recognition program. \textit{Ondemand}'s sampling rate is set to 100 ms.
The system sends a request once every second, i.e., the deadline for one request is 1000 ms.
With the highest frequency (1.48GHz), one request takes about 350 ms to complete.

It is worth mentioning that, as of now, only some high-end CPU series support per-core DVFS, which means that each core runs at a different frequency.
For CPUs without per-core DVFS support, the entire CPU package must run at the same V/f.
In this case, although the Jetson Nano Board supports a quad-core CPU, built-in governors will adjust the frequency according to the highest utilization of all the cores (green bar in the plot).

\begin{figure}
	\centering
	\includegraphics[width=0.5\textwidth]{images/6.png}
	\caption{\textit{Ondemand} will try to reduce the CPU frequency in low utilization periods.}
	\label{fig:6}
\end{figure}

\textit{Ondemand} is effective in its ability to save energy by reducing frequency when utilization is low, as shown in Fig.~\ref{fig:6}.
The reduced voltage with frequency saves both dynamic and static energy consumption.
Being able to reduce the frequency when the system is idle can effectively save energy.

\begin{figure}
	\centering
	\includegraphics[width=0.5\textwidth]{images/5.png}
	\caption{Energy waste (top) and performance loss (bottom) caused by \textit{Ondemand}'s tuning.}
	\label{fig:5}
\end{figure}

The energy saving is not completely free. \textit{Ondemand}'s tuning can also hurt the performance.
It predicts the demand in a future period to be the same as the demand in a past period (lines 5-9 in algorithm 1), which means the tuning is always one period slower.
Specifically, when workload transitions from CPU idle periods to CPU intensive periods, \textit{Ondemand} will inevitably set a low frequency at the beginning of the intensive periods (as shown in Fig.~\ref{fig:5}).
However, \textit{Ondemand} is able to set high CPU frequencies in consecutive CPU intensive periods.

\textit{Ondemand} can waste energy compared to a perfect frequency tuning strategy.
The reason is the same as discussed above: it is always one period slower.
As shown in Fig.~\ref{fig:5}, \textit{Ondemand} could set high frequencies in some low utilization periods.
Obviously, the smaller the period, the more opportunities for \textit{Ondemand} regulation, and the smaller the loss from an unwise tuning.

Overall, as long as your computing needs are not extremely latency intensive, turning on \textit{Schedutil} or \textit{Ondemand} governor can save you power overhead at the cost of little performance loss.

\subsection{Tune the Trade Off between Performance and Energy}

The default settings of \textit{Ondemand} discussed above can be seen as energy saving with as little performance loss as possible.
This is the same for \textit{Schedutil}.
When demand permits further performance reductions, further frequency reductions to save more energy become possible, which is also an characteristic of embedded systems.
As shown in Fig.~\ref{fig:4}, since the system only sends one request per 1 s, a slack of 0.75 s occurs at the default setting.
In this scenario, we would want to adjust the tuning policy to fill the slack.

As of V 5.13,  \textit{Ondemand} is the only governor that provides a service that can intuitively tune the trade off between performance and energy.
It is worth mentioning that when using \textit{Ondemand} for comparison, many works use only the initial settings of \textit{Ondemand}, neglecting its function of tuning trade off.
The trade off is done by a tunable parameter: \textit{powersave\_bias}, which logically belongs to [0, 1].
\textit{Ondemand} will use this bias to make a discount to the calculated frequency (line 10 in algorithm 1).
The higher the bias, the greater the discount.

\begin{figure}
	\centering
	\includegraphics[width=0.5\textwidth]{images/7.jpg}
	\caption{\textit{Ondemand} tuning when \textit{powersave\_bias}=0, 0.3, 0.6}
	\label{fig:7}
\end{figure}

This simple method allows for efficient selection of lower frequencies to fill the slack.
When the CPU offers fine-grained frequency options, this method can be used to find a solution that is good enough to meet the performance requirements.
As shown in Fig.~\ref{fig:7}, by tuning the \textit{powersave\_bias}, \textit{Ondemand} gradually reduces the upper limit of the frequency.

